Energy exchanges between coherent modes in the near wake of a rotor model at different tip speed ratios

In this work we investigate the spatio-temporal nature of various coherent modes present in a rotor wake using a combination of new PIV experiments and data from Biswas and Buxton (2024). A multi-scale triple decomposition of the acquired velocity field is sought to extract the coherent modes and thereafter, the energy exchanges to and from them are studied using the multi-scale triple-decomposed coherent kinetic energy budgets developed by Baj and Buxton (2017). Different frequencies forming the tip vortex system (such as the blade passing frequency, turbine's rotational frequency and their harmonics) are found to be energised by different sources such as production from the mean flow or non-linear triadic interaction or both, similar to the primary, secondary or the mixed modes discussed in Biswas et al. (2022). In fact, the tip vortex system forms a complex network of nonlinear triadic energy transfers, the nature and the magnitudes of which depend on \lambda. On the other hand, the modes associated with the sheddings from the nacelle or tower and wake meandering are found to be primarily energised by the mean flow. We show that the tip vortex system exchanges energy with the mean flow primarily through the turbine's rotational frequency. In fact, the system transfers energy back to the mean flow through the turbine's rotational frequency at some distance downstream marking the onset location of wake recovery (x_{wr}). x_{wr} is shown to reduce with \lambda due to stronger interaction and earlier merging of the tip vortices at a higher \lambda.

==> README <==

  The ulem package provides various types of underlining that can stretch
  between words and be broken across lines in LaTeX or plain TeX.
  In LaTeX ulem replaces italics with underlining in \em-phasized text.
  A declaration of \normalem (or the \usepackage option "normalem") restores 
  the normal \em and \emph behavior.

  Copyright 1989-2019 by Donald Arseneau (Vancouver, Canada; asnd@triumf.ca)

  This software may be freely transmitted, reproduced, or modified for any
  purpose provided that this copyright notice is left intact.  

